Semi-supervised Contrastive Learning for Label-efficient Medical Image Segmentation

The success of deep learning methods in medical image segmentation tasks heavily depends on a large amount of labeled data to supervise the training. On the other hand, the annotation of biomedical images requires domain knowledge and can be laborious. Recently, contrastive learning has demonstrated great potential in learning latent representation of images even without any label. Existing works have explored its application to biomedical image segmentation where only a small portion of data is labeled, through a pre-training phase based on self-supervised contrastive learning without using any labels followed by a supervised fine-tuning phase on the labeled portion of data only. In this paper, we establish that by including the limited label in formation in the pre-training phase, it is possible to boost the performance of contrastive learning. We propose a supervised local contrastive loss that leverages limited pixel-wise annotation to force pixels with the same label to gather around in the embedding space. Such loss needs pixel-wise computation which can be expensive for large images, and we further propose two strategies, downsampling and block division, to address the issue. We evaluate our methods on two public biomedical image datasets of different modalities. With different amounts of labeled data, our methods consistently outperform the state-of-the-art contrast-based methods and other semi-supervised learning techniques.

==> subsection/related_works.tex <==
One track of related works to this paper is about how to tackle the problem of limited annotated data for medical image segmentation. 
We classify those works into two groups.
\textbf{Data augmentation} tries to enlarge the dataset with the synthesized image and labels.
For example,\cite{bowles2018gan} demonstrated improved performance in brain segmentation tasks after introducing GAN derived data to training set.
\cite{chaitanya2019semi} used GAN to model the image transformation and also leveraged unlabeled dataset for generating data. 
\textbf{Semi-supervised learning} takes advantage of the unlabeled data for additional information during training. 
Self-training \cite{bai2017semi} updated models parameters after being trained with labeled and unlabeled data alternatively.
~\cite{zhang2017deep, li2020shape} introduced an adversarial network to distinguish segmentation result between images with annotations and without annotations so that the segmentation network finally generated segmentation of the same quality for the unlabeled data.
Most recently, TCSM\cite{li2020transformation} added a regularization loss to encourage the segmentation result of the same unlabeled data after different perturbations to be the same.

\textbf{Contrastive learning} belongs to pretext task and it is originally employed to learn image features that boost the subsequent classification task under self-supervised setting. 
\cite{chen2020simple} forced the embedding features of an image to be similiar with that of the image after several transformations and dissimilar to all other images in the mini-batch in latent space.
\cite{he2020momentum} built an dynamic queue and a moving-averaged encoder to increase the negative pairs in the batch.
In terms of medical image segmentation, as far as we are aware, there are few works employing contrastive learning, including\cite{chaitanya2020contrastive, li2020contrastive}. \cite{li2020contrastive} added the contrastive loss to the cross entropy loss for joint training and was not targeted for limited annotation problem. 
